What Do Self-Supervised Speech Models Know About Words?

Many self-supervised speech models (S3Ms) have been introduced over the last few years, improving performance and data efficiency on various speech tasks. However, these empirical successes alone do not give a complete picture of what is learned during pre-training. Recent work has begun analyzing how S3Ms encode certain properties, such as phonetic and speaker information, but we still lack a proper understanding of knowledge encoded at the word level and beyond. In this work, we use lightweight analysis methods to study segment-level linguistic properties -- word identity, boundaries, pronunciation, syntactic features, and semantic features -- encoded in S3Ms. We present a comparative study of layer-wise representations from ten S3Ms and find that (i) the frame-level representations within each word segment are not all equally informative, and (ii) the pre-training objective and model size heavily influence the accessibility and distribution of linguistic information across layers. We also find that on several tasks -- word discrimination, word segmentation, and semantic sentence similarity -- S3Ms trained with visual grounding outperform their speech-only counterparts. Finally, our task-based analyses demonstrate improved performance on word segmentation and acoustic word discrimination while using simpler methods than prior work.

==> figs/awd-other.tex <==
\begin{figure}[ht]
\begin{minipage}[b]{1.0\linewidth}
\small

 \centering
 \centerline{\includegraphics[width=8cm, trim=0 305 0 0, clip]{images/legend3.pdf}}
\end{minipage}
\begin{minipage}[b]{1.0\linewidth}

\centering
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 130 0 60, clip]{images/awe_other_small.pdf}
         \caption{Acoustic word discrimination results using mean-pooled S3M word segment representations on LibriSpeech dev-other.}
         \label{fig:awe-other}
     \end{subfigure}

     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 130 0 60, clip]{images/dtw_other_small.pdf}
         \caption{Acoustic word discrimination results using DTW between frame-level S3M word segment representations on LibriSpeech dev-other.}
         \label{fig:dtw-other}
     \end{subfigure}
\end{minipage}
\vspace{-0.3cm}
\caption{\it Acoustic word discrimination results on dev-other}
  \label{fig:dev-other}
\vspace{-0.3cm}
\end{figure}

==> figs/res1-large.tex <==
\begin{figure}[t]
\begin{minipage}[b]{1.0\linewidth}
\small

 \centering
 \centerline{\includegraphics[width=8cm, trim=0 275 0 0, clip]{images/legend-scores-large.pdf}}
\end{minipage}
\begin{minipage}[b]{1.0\linewidth}

\centering
     % \hfill
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 5 0 200, clip]{images/cca_cd_word_small.pdf}
         \caption{Word identity as measured via CCA similarity between S3M word segment representations and one-hot vectors.}
         \label{fig:cca-word-large}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 5 0 200, clip]{images/awe_clean_small.pdf}
         % \includegraphics[width=\linewidth, trim=0 5 0 200, clip]{images/awe_other_small.pdf}
         \caption{Acoustic word discrimination results using mean-pooled S3M word segment representations on LibriSpeech dev-clean.\ap{dev-other plot command commented}}
         \label{fig:awe-clean-large}
     \end{subfigure}
     
     % \begin{subfigure}[b]{\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth, trim=0 5 0 210, clip]{images/dtw_clean_small.pdf}
     %     \caption{Acoustic word discrimination results using DTW between frame-level S3M word segment representations on LibriSpeech dev-clean.}
     %     \label{fig:dtw-clean}
     % \end{subfigure}
     
     % \begin{subfigure}[b]{\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth, trim=0 130 0 60, clip]{images/awe_other_small.pdf}
     %     \caption{Word discrimination results using AWE on test-other.}
     %     \label{fig:awe-other}
     % \end{subfigure}

     % \begin{subfigure}[b]{\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth, trim=0 130 0 60, clip]{images/dtw_other_small.pdf}
     %     \caption{Word discrimination results using DTW on test-other.}
     %     \label{fig:dtw-other}
     % \end{subfigure}
\end{minipage}
\vspace{-0.3cm}
\caption{\it Measure of different word-level pronunciation for large models via (a) comparison with AGWE and (b-c) evaluation on acoustic word discimination.
\todo{to be displayed next to \fig~\ref{fig:scores1-small}}
}
  \label{fig:scores1-large}
\vspace{-0.3cm}
\end{figure}

==> figs/res1-small.tex <==
\begin{figure}[t]
\begin{minipage}[b]{1.0\linewidth}
\small

 \centering
 \centerline{\includegraphics[width=8cm, trim=0 275 0 0, clip]{images/legend-scores-small.pdf}}
\end{minipage}
\begin{minipage}[b]{1.0\linewidth}

\centering
     % \hfill
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 145 0 60, clip]{images/cca_cd_word_small.pdf}
         \caption{Word identity as measured via CCA similarity between S3M word segment representations and one-hot vectors.}
         \label{fig:cca-word-base}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 145 0 60, clip]{images/awe_clean_small.pdf}
         % \includegraphics[width=\linewidth, trim=0 145 0 60, clip]{images/awe_other_small.pdf}
         \caption{Acoustic word discrimination results using mean-pooled S3M word segment representations on LibriSpeech dev-clean.\ap{dev-other plot command commented}}
         \label{fig:awe-clean-base}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 145 0 60, clip]{images/dtw_clean_small.pdf}
         % \includegraphics[width=\linewidth, trim=0 145 0 60, clip]{images/dtw_other_small.pdf}
         \caption{Acoustic word discrimination results using DTW between frame-level S3M word segment representations on LibriSpeech dev-clean.\ap{dev-other plot command commented}}
         \label{fig:dtw-clean}
     \end{subfigure}
     
     % \begin{subfigure}[b]{\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth, trim=0 130 0 60, clip]{images/awe_other_small.pdf}
     %     \caption{Word discrimination results using AWE on test-other.}
     %     \label{fig:awe-other}
     % \end{subfigure}

     % \begin{subfigure}[b]{\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth, trim=0 130 0 60, clip]{images/dtw_other_small.pdf}
     %     \caption{Word discrimination results using DTW on test-other.}
     %     \label{fig:dtw-other}
     % \end{subfigure}
\end{minipage}
\vspace{-0.3cm}
\caption{\it Measure of different word-level pronunciation for small models via (a) comparison with AGWE and (b-c) evaluation on acoustic word discimination.
\todo{to be displayed next to \fig~\ref{fig:scores1-large}}
}
  \label{fig:scores1-small}
\vspace{-0.3cm}
\end{figure}

==> figs/res2-large.tex <==
\begin{figure}[t]
\begin{minipage}[b]{1.0\linewidth}
\small

 \centering
 \centerline{\includegraphics[width=8cm, trim=0 275 0 0, clip]{images/legend-cca-large.pdf}}
\end{minipage}
\begin{minipage}[b]{1.0\linewidth}

\centering
\ifdraft
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 5 0 200, clip]{images/cca_cd_phone_small.pdf}
         \caption{\ap{CCA-phone for the purpose of comparison}}
         \label{fig:cca-phoneL}
     \end{subfigure}
\fi     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 5 0 200, clip]{images/cca_cd_agwe_small.pdf}
         \caption{Word pronunciation content, as measured via CCA similarity between S3M word segment representations and AGWEs}
         \label{fig:agweL}
     \end{subfigure}

 \ifdraft
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 10 0 195, clip]{images/cca_cd_word_small.pdf}
         \caption{\ap{CCA-word for the purpose of comparison}}
     \end{subfigure}
\fi     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 10 0 195, clip]{images/cca_cd_syntactic_small.pdf}
         \caption{Syntactic content as measured via CCA similarity between S3M word segment representations and POS attributes.}
         \label{fig:ptbL}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 10 0 195, clip]{images/cca_cd_semantic_small.pdf}
         \caption{Semantic content as measured by CCA similarity between S3M word segment representations and SemCor attributes.}
         \label{fig:semcorL}
     \end{subfigure}

\ifdraft
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 10 0 195, clip]{images/cca_cd_glove_small.pdf}
         \caption{Semantic content as measured by CCA similarity between S3M word segment representations and GloVe.}
         \label{fig:gloveL}
     \end{subfigure}
\fi     

     % \begin{subfigure}[b]{\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth, trim=0 130 0 60, clip]{images/spoken_sts_small.pdf}
     %     \caption{Performance on spoken STS task.}
     %     \label{fig:sts}
     % \end{subfigure}

     % \begin{subfigure}[b]{\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth, trim=0 155 0 45, clip]{images/word-seg.png}
     %     \caption{\ap{Filler for unsupervised word segmentation results}}
     %     \label{fig:glove}
     % \end{subfigure}
\end{minipage}
\vspace{-0.3cm}
\caption{\it Measure of different linguistic properties for large S3Ms using CCA, where the shaded area corresponds to values across five different runs.
\todo{To-be-displayed next to \fig~\ref{fig:cca-scores-small}
\ap{Re-think if we want to include both SemCor and GloVe here; and if so, what different information are we learning from each?}}
}
  \label{fig:cca-scores-large}
\vspace{-0.3cm}
\end{figure}

==> figs/res2-small.tex <==
\begin{figure}[t]
\begin{minipage}[b]{1.0\linewidth}
\small

 \centering
 \centerline{\includegraphics[width=8cm, trim=0 275 0 0, clip]{images/legend-cca-small.pdf}}
\end{minipage}
\begin{minipage}[b]{1.0\linewidth}

\centering
\ifdraft
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 145 0 60, clip]{images/cca_cd_phone_small.pdf}
         \caption{\ap{CCA-phone for the purpose of comparison}}
         \label{fig:cca-phoneB}
     \end{subfigure}
\fi     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 145 0 60, clip]{images/cca_cd_agwe_small.pdf}
         \caption{Word pronunciation content, as measured via CCA similarity between S3M word segment representations and AGWEs}
         \label{fig:agweB}
     \end{subfigure}

 \ifdraft
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 145 0 60, clip]{images/cca_cd_word_small.pdf}
         \caption{CCA-word \ap{for the purpose of comparison}}
     \end{subfigure}
 \fi
 
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 145 0 60, clip]{images/cca_cd_syntactic_small.pdf}
         % \includegraphics[width=\linewidth, trim=0 130 0 75, clip]{images/cca_cd_syntactic_small.pdf}
         \caption{Syntactic content as measured via CCA similarity between S3M word segment representations and POS attributes.}
         \label{fig:ptbB}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 145 0 60, clip]{images/cca_cd_semantic_small.pdf}
         \caption{Semantic content as measured by CCA similarity between S3M word segment representations and SemCor attributes.}
         \label{fig:semcorB}
     \end{subfigure}
 \ifdraft    
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 145 0 60, clip]{images/cca_cd_glove_small.pdf}
         \caption{Semantic content as measured by CCA similarity between S3M word segment representations and GloVe.}
         \label{fig:gloveB}
     \end{subfigure}
\fi        
     % \begin{subfigure}[b]{\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth, trim=0 130 0 75, clip]{images/spoken_sts_small.pdf}
     %     \caption{Performance on spoken STS task.}
     %     \label{fig:sts}
     % \end{subfigure}

     % \begin{subfigure}[b]{\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth, trim=0 155 0 45, clip]{images/word-seg.png}
     %     \caption{\ap{Filler for unsupervised word segmentation results}}
     %     \label{fig:glove}
     % \end{subfigure}
\end{minipage}
\vspace{-0.3cm}
\caption{\it Measure of different linguistic properties for small S3Ms using CCA, where the shaded area corresponds to values across five different runs.
\todo{to be displayed next to \fig~\ref{fig:cca-scores-large}}
\ap{Re-think if we want to include both SemCor and GloVe here; and if so, what different information are we learning from each?}
}
  \label{fig:cca-scores-small}
\vspace{-0.3cm}
\end{figure}

==> tables/nn.tex <==
\begin{table}[h]
\small
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lll}
\hlineB{2}
\begin{tabular}[c]{@{}l@{}}Embedding\\ map\end{tabular}         & Word   & Nearest neighbors                                       \\\hlineB{2}
\multirow{2}{*}{SemCor} & 
family &
\begin{tabular}[c]{@{}l@{}}government, leaders, elite, platoon\end{tabular}        \\
                        & mix    &
\begin{tabular}[c]{@{}l@{}}flourish, merge, adapt, intensify, started \end{tabular}      \\\hline
                        % & hamper & cure, can, fuse, mold, die, reverse, widen, recur       \\\hline
\multirow{2}{*}{GloVe}  & family & 
\begin{tabular}[c]{@{}l@{}}husband, father, mother, sister, wife \end{tabular}\\
                        & mix    & 
\begin{tabular}[c]{@{}l@{}}mixture, blend, combine, butter, stir, jam   \end{tabular}    \\\hlineB{2}
                        % & hamper & undermine, basket, dampen, complicate, disrupt     \\\hlineB{2}    
\end{tabular}
}
\caption{Nearest neighbors in terms of cosine similarity between SemCor and GloVe embeddings. \ap{candidate for removal, an example can be incorporated in the text.}}
\label{tab:nn}
\end{table}

==> tables/ptb.tex <==
\begin{table}[h]
\small
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llllll}
\textbf{WORD} & \textbf{PTB.NN} & \textbf{PTB.NNP} & \textbf{PTB.VB} & $\cdots$ & \textbf{PTB.JJ} \\\hlineB{2}
spring        & 0.94       & 0.037     & 0.02            &    $\cdots$          & 0.00            \\
fall          & 0.49        & 0.00    & 0.43            &     $\cdots$         & 0.00            \\
light         & 0.52        & 0.046    & 0.02            &   $\cdots$           & 0.41           
\end{tabular}
}
\caption{Examples of syntactic attribute vectors, constructed using PTB~\cite{tsvetkov2016correlation}. \ap{candidate for removal.}}
\label{tab:ptb}
\end{table}

==> tables/semcor.tex <==
\begin{table}[h]
\centering
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
 {\bf WORD}            & {\bf NN.GROUP} & {\bf NN.ACT} & $\cdots$ & {\bf VB.CHANGE} \\\hlineB{2}
family       & 0.958        & 0.042 & $\cdots$           & 0        \\
mix          & 0          &  0     & $\cdots$          & 0.909    \\
% headquarters & 0.1     & 0         & 0     & ... & 0.900      & 0        \\
industry     & 0.792        & 0.208 & $\cdots$          & 0       
% hamper     & 0   & 0.666         & 0 & $\cdots$        & 0 
\end{tabular}
}
\caption{Examples of semantic attribute vectors, constructed using SemCor~\cite{tsvetkov2015evaluation}.\ap{candidate for removal, an example can be incorporated in the text.}}
\label{tab:semcor}
\end{table}

==> tables/sts.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lc}
\hlineB{2}
\textbf{Sentence pairs}                                                                                                                               & \textbf{\begin{tabular}[c]{@{}c@{}}Human similarity judgement\\ (between 0 and 5)\end{tabular}} \\\hlineB{2}
\begin{tabular}[c]{@{}l@{}}police arrested 2 honduran drug trafficking suspects\\ bulgarian police arrest head of drug trafficking group\end{tabular} & 1.4                                                                                             \\[10pt]
\begin{tabular}[c]{@{}l@{}}cyprus bailout remarks alarm markets\\ why cyprus bailout is nothing more than usual euro nonsense\end{tabular}            & 2.6                                                                                             \\[10pt]
\begin{tabular}[c]{@{}l@{}}former alaska gov sarah palin is no long a commentator for fox news\\ fox news and sarah palin part ways\end{tabular}      & 4.4          \\\hlineB{2}                                                                                  
\end{tabular}
\caption{Example sentence pairs from the STS data.
\ap{candidate for removal}
}
\label{tab:sts}
\end{table*}
